Individually Fair Ranking

We develop an algorithm to train individually fair learning-to-rank (LTR) models. The proposed approach ensures items from minority groups appear alongside similar items from majority groups. This notion of fair ranking is based on the definition of individual fairness from supervised learning and is more nuanced than prior fair LTR approaches that simply ensure the ranking model provides underrepresented items with a basic level of exposure. The crux of our method is an optimal transport-based regularizer that enforces individual fairness and an efficient algorithm for optimizing the regularizer. We show that our approach leads to certifiably individually fair LTR models and demonstrate the efficacy of our method on ranking tasks subject to demographic biases.

==> YK-macros.tex <==

\def\Avar{{\sf Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{{\sf aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{{\sf avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{{\sf bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{{\sf Ber}}
\def\bin{{\sf bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{{\sf cat}}
\def\Cov{{\sf Cov}}
\def\cov{{\sf cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{{\sf cl}}
\def\complex{{\bbC}}
\def\cone{{\sf cone}}
\def\conv{{\sf conv}}
\def\deq{\overset{d}{=}}
\def\det{{\sf det}}
\def\diag{{\sf diag}}
\def\diam{{\sf diam}}
\def\dist{{\sf dist}}
\def\dom{{\sf dom}}
\def\doop{{\sf do}}
\def\dto{\overset{\sf d}{\to}}
\def\Ex{{\bbE}}
\def\Exp{{\sf Exp}}
\def\exp{{\sf exp}}
\def\eg{{\it e.g.}}
\def\epi{{\sf epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\iid{{\sf iid}}
\def\ind{{\sf ind}}
\def\intr{{\sf int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{{\sf KL}}
\def\ker{{\sf ker}}
\def\lspan{{\sf span}}
\def\maximize{{\sf maximize}}
\def\med{{\sf med}}
\def\minimize{{\sf minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{{\sf Poi}}
\def\Pr{{\bbP}}
\def\peq{\overset{\sf p}{=}}
\def\plim{{\sf plim}}
\def\proj{{\sf proj}}
\def\prox{{\sf prox}}
\def\pto{\overset{\sf p}{\to}}
\def\ran{{\sf ran}}
\def\rank{{\sf rank}}
\def\reals{{\bbR}}
\def\relint{{\sf relint}}
\def\sign{{\sf sign}}
\def\supp{{\sf supp}}
\def\symm{{\bbS}}

\def\st{\textrm{subject to}}
\def\tr{{\sf tr}}
\def\tube{{\sf tube}}
\def\TV{{\sf TV}}
\def\unif{{\sf unif}}
\def\Var{{\sf Var}}
\def\var{{\sf var}}
\def\vct{{\sf vec}}
\def\veps{\varepsilon}
\def\vol{{\sf vol}}
\def\zeros{\mathbf{0}}


==> YK-thm-macros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}


==> amanda/data.tex <==
1. Yahoo Learning to Rank: http://proceedings.mlr.press/v14/chapelle11a/chapelle11a.pdf?

2. W3C experts in \cite{DBLP:journals/corr/abs-1805-08716}, need to request. They inferred gender by looking at the name manually and injected bias by placing qualified men before qualified women. But then I don't understand how they estimated the probability that a document is in the first position, unless the probability is either 1 or 0. 

3. Engineering Student data set in \cite{DBLP:journals/corr/abs-1805-08716}, need to request. They turned it into a LTR dataset by sorting by grade.

4. Law Students Data set in \cite{DBLP:journals/corr/abs-1805-08716}. They turned it into a LTR dataset.

5. XING Data set in \cite{zehlike2017fa}. ``XING is a career-oriented website from which we automatically collected the top-40 profiles returned for 54 queries, using three for which there is a clear difference between top-10 and top-40. We used a non-personalized (not logged in) search interface and confirmed that it yields the same results from different locations. For each profile, we collected gender, list of positions held, list of education details, and the number of times each profile has been viewed in the platform, which is a measure of popularity of the profile. With this information, we constructed an ad-hoc score: the months of work experience plus the months of education, multiplied by the number of views of the profile. This score tends to be somewhat higher for profiles in the first positions of the search results, but in general does not approximate the proprietary ordering in which profiles are shown. We include this score and its components in our anonymized data release. We use the appropriate gender for each query as the protected group." Code and data: https://github.com/MilkaLichtblau/FA-IR_Ranking

6. Airbnb dataset used in \cite{biega2018equity}. http://insideairbnb.com/

7. Stackexchange data set used in \cite{biega2018equity}

8. TREC 2019 Fair Ranking Track \cite{biega2020overview}: The data is based on Semantic Scholar searches.
- paper data: paper ID, title, abstract, authors (resolved to author IDs), inbound and outbound citations, sensitive feature is whether or not authors are from an advanced economy country, developing, or mixed (ie authors from both advanced and developing country)
- query data: query string, query normalized frequency, a list of documents with number of clicks each document gets (only 6 documents per query, unless the documents presented for a given query change over time and I’m not sure if the documents are ordered or just presented as a set), binary relevance (if a document was clicked or not)
- lots of issues: click rate could be biased, binary relevance, can’t use gender, the fact that it’s only 6 documents might make it trivial


==> amanda/intro.tex <==
Ranking systems are ubiquitous.

\cite{geyik2019fairness} empirically showed that LinkedIn queries are not group fair. Interestingly, they showed that group fairness does not necessarily harm business metrics.

==> amanda/related_work_summary.tex <==
%Another line of work models the amount of exposure documents receive at each position in the ranking and allocates exposure based on this exposure model and document relevance \cite{singh2018Fairness, DBLP:journals/corr/abs-1805-08716, biega2018equity, singh2019Policy}. These works consider both group and individual fairness settings. \cite{DBLP:journals/corr/abs-1805-08716} learns a group fair LTR system that gives the minority group at least as much as exposure as the majority group. Similarly, \cite{singh2019Policy}, which builds on the post-processing work of \cite{singh2018Fairness}, learns a group fair or individually fair LTR system using a similar constraint that also takes relevance into account. \cite{biega2018equity} considers the online setting and proposes a post processing algorithm to obtain an individually fair LTR system by requiring that the ratio of cumulative attention to cumulative relevance is equal for each document.

\cite{StoyanovichAndYang} propose three group fairness measures. In their set-up, they assume a binary protected attribute. However, they do not assume a relevance score of each item, so their notions of fairness are not tied to any notion of accuracy. Their first two metrics define a fair ranking as a ranking that for the first $k$ positions in the ranking for $k \in [k_1, k_2, ...]$, the proportion of individuals from the majority/minority group is approximately equal to the proportion of majority/minority in the whole population. Their metrics put more importance of the proportions being equal for smaller $k$. The difference between the first two metrics is one is differentiable version of the other. Their third metric looks at the ratio of the majority to the minority in the top $k$ compared to the ratio of the majority to the minority. This paper is mostly about proposing metrics, not learning a fair ranking system although they do have some preliminary experiments by using their definitions of fairness as regularizer. 

\cite{DBLP:journals/corr/abs-1805-08716} propose a list-wise fair LTR algorithm: DELTR (Disparate Exposure in Learning to Rank). They claim that they are the first to propose an in-processing fair LTR algorithm. They assume that each document belongs to a minority or majority group. Their notion of fairness borrows from the definition of exposure in \cite{singh2018fairness}: \[\mathrm{Exposure}(d|P) = \sum_{i=1}^n P_{d,j} v_j\] where $d$ is a document, $P_{d,j}$ is the probability that $d$ is ranked in position $j$, and $v_j$ is the position bias of position $j$ ($v_j = \frac{1}{\log(1+j)}$). However, they only consider the case when $j = 1$ because their loss function only depends on the probability of a document being ranked first. They use a group notion of fairness: for each query, the average exposure documents from the minority group receive should equal or exceed the exposure that documents from the majority group receive. They incorporate this fairness constraint as a regularizer to the ListNet objective. 

%But how do you compute the empirical probability that a document is the first? With the relevance scores? What does the data for their real experiments look like? For the engineering student data set, are there only like 16 training samples and 4 testing samples?

\cite{zehlike2017fa} they propose a definition of group fairness for rankings, give a statistical test for determining if a ranking is fair, and propose a post-processing method to obtain a fair ranking. Post-processing means that they do not learn scores for each document and use the relevance scores given to them, i.e. they do not learn a ranking system which can take as input new queries/documents and predict new rankings. Their notion of fairness ``is based on ensuring that the proportion of protected candidates in every prefix of the top-$k$ ranking remains statistically above or indistinguishable from a given minimum." They assume a binary protected attribute. Their post-processing algorithm is a greedy algorithm to produce a top-$k$ fair ranking by separately sorting the majority/minority group into two lists based on relevance scores. Based on their statistical test, for each $t \in [k]$, there must be at least $p_t$ minority individuals in the top $t$ of the ranking. Therefore, to pick the $t$-th individual in the ranking of size $k$, they either pick the best individual remaining from the union of the majority/minority lists or they must pick the best individual remaining from the minority list if the number of minority individuals will not exceed $p_t$.

\cite{biega2018equity} proposes an individually fair definition of fairness in rankings: amortized over multiple queries, the attention (measured by the position in the ranking) each document receives should be proportional to its relevance. They refer to this definition is \textit{equity of attention}. This is their motivation: ``For example, attention could decrease geometrically, whereas relevance scores may decrease linearly as the rank decreases. If a ranking is displayed unchanged to many searchers over time, the lower-ranked subjects might be systematically and repeatedly disadvantaged in terms of the attention they receive." This is the same idea in \cite{singh2019Policy} except \cite{biega2018equity} consider the individual fairness, online setting. These works were written in parallel. They propose a post-processing algorithm to attain rankings that satisfy amortized individual fairness by considering an online integer linear program (ILP), but they do not propose an efficient or optimal algorithm to solve the ILP.

\cite{DBLP:journals/corr/CelisSV17} consider the problem of finding a utility maximizing ranking subject to upper and lower bounds on the number of documents belonging to a group that appear in the first $k$ positions for $k \in K$. They assume knowledge of the utility that a document in a certain position contributes to a ranking. Their algorithm is a post-processing technique. The main results of their paper are ``fast, exact and approximation algorithms for this constrained ranking maximization problem along with complementary hardness results which, together, give a solid understanding of the computational complexity of this problem." This paper is very TCS and has no experiments.

\cite{singh2018Fairness} propose an exposure based definition of fairness and a post-processing algorithm. In particular, they show how to maximize utility subject to fairness constraints as a linear program where instead of finding a single ranking, they find a distribution of rankings to make the problem feasible. To switch from a single ranking to distributions of rankings, they look at doubly stochastic matrices since every ranking corresponds to a doubly stochastic matrix and vice versa. As the motivation for their exposure based fairness definition, they show that a small difference in relevance can lead to a large difference of exposure, which is particularly important for the application of who to hire for a job. They propose 3 definitions of exposure based fairness. First, demographic parity ensures that the exposure of both groups are equal. Second, disparate treatment ensures the exposure of both groups are proportional to their utility. Third, disparate impact ensures that the click through rates (as a function of exposure) is proportional to utility.

\cite{singh2019Policy} 

\cite{geyik2019fairness} proposes group fair measures very similar to \cite{StoyanovichAndYang}. Their notion of a fair ranking is one whose top $k$ positions contain a certain proportion of individuals from the minority group. The measures they propose are (1) skew\@k and (2) normalized discounted cumulative KL-divergence.  Skew\@k for a sensitive feature is the log of the ratio of the proportion of individuals in the top-k positions with that sensitive feature over the desired proportion.  Normalized discounted cumulative KL-divergence is like normalized discounted cumulative gain except the KL divergence between the distribution of the number of individuals from each sensitive group in the top $k$ positions and the desired distribution is used instead of relevance. They provide a post-processing algorithms, one of which is similar to \cite{zehlike2017fa}. The most interesting thing about this work is that they deployed their algorithm on LinkedIn and found that post-processing the rankings to obtain gender group fair rankings did not effect the quality of the rankings (measured by the number of recruiter messages sent and accepted by candidates) from the user perspective. Group fairness measures were improved 3x and 95\% of all searches had the appropriate gender balance.  

\cite{sapiezynski-2019-fairness} proposes a group fairness metric and a statistical test to audit a ranking for fairness. Their definition/audit depends on the distribution of exposure each sensitive group receives compared to an ideal distribution. Their work is what they claim is a more accurate model of exposure than the model used in \cite{singh2018Fairness, singh2019Policy, biega2018equity}. In particular, they claim that modeling user attention with inverse log weights (i.e. 1/log(i)) is inappropriate because it does not attribute enough attention to the top of the ranking and because it assumes that ``user behavior is the static across all platforms and for all search queries.”

\cite{10.1145/3299869.3300079} work is quite different from the rest. They consider the setting where the ranking function is linear and given by a human. Their goal is to help a human choose positive linear weights that result in quality rankings (ie as close to the original weights that the human gave) yet satisfy fairness constraints given by an oracle. They focus on group fairness but their framework is applicable to arbitrary fairness constraints.

\cite{10.1145/3308558.3313443} propose new definitions of fair rankings that extend beyond exposure and minority representation in the top-k. Their work also addresses the whole ranking instead of just the top-k positions. Their setting is different from the standard LTR setting since they assume their is an underlying ground truth ranking in contrast to relevance scores for the items and their measures use concordant and discordant pairs..``We define a new set of fairness criteria customized for rankings: Rank Equality, Rank Calibration, and Rank Parity based on novel rank-specific error metrics. These criteria are model-agnostic and applicable for many ranking applications, capturing key notions of fairness previously applied only for classification.”  Rank Equality tries to define the false negative rate in classification equivalent for ranking which is a function of discordant pairs where the minority group was incorrectly ranked worse. Rank Calibration of a group tries to define calibration for rankings as a function of the number of discordant pairs where at least one item is from that group. Rank Parity is a function of how many disconcordant pairs ranks an item from one group over another.
discordant

\cite{10.1145/3351095.3372858} consider the scenario where the observed relevance scores for one group is biased, and propose enforcing constraints of the form ``there needs to be at least $\alpha_{k,g}$ individuals from group $g$ in the top $k$ of the ranking.” They assume each item $i$ has a true relevance score $w_i$, but that the observed relevance scores are biased for each group $g$, that is the observed relevance for item $i$ is $\beta_g w_i$, where $\beta_g \geq 0$. Their goal is to find a ranking that maximizes utility as a function of the true relevance scores. Theoretically, they have three results. First, they show that there always exists constraints (i.e. minimums on the number of individuals from group $g$ in the top $k$ positions) so that the ranking that maximizes the constrained problem based on the observed biased relevance scores equals the ranking that maximizes the utility based on the true relevance scores. However, these constraints require knowing the bias, i.e. $\beta_g$. Second, they show that if the relevance scores for both groups are drawn from the same continuous distribution, then with high probability the optimal ranking based on the true relevances scores puts $k \frac{m_a}{m_a m_b}$ individuals from the minority group in the top k positions where $m_a$ is the number of minority items and $m_b$ is the number of majority candidates. This motivates enforcing a ``Rooney Rule” type of constraint, i.e. require that at least $k \frac{m_a}{m_a m_b}$ of the individuals in the top $k$ come from the minority. Third, assuming that the distribution that the utilities are drawn from is uniform, then maximizing utility subject to the ``Rooney Rule” type of constraints produces a ranking whose utility under the true relevances is close to the utility maximizing ranking based on the true, unbiased relevances.

\cite{0d8212cdb710458e9a32312c0ffe3a11} consider the problem of group fairness when each person can belong to more than one group. Their notion of fairness is that anyone in the top $k$ from group $g$ must have a higher relevance than anyone not in the top $k$ in group $g$. There exists cases when maximizing utility subject to fairness (what they call diversity) constraints of the form “there must be at least $\alpha_{k,g}$ of people from group $g$ in the top $k$ for the ranking” results in a ranking that violates this notion of fairness. See their example 1. This cannot happen with just two groups (e.g. male and female). They propose an integer program to find a ranking that satisfies both their notion of fairness and diversity constraints.

\cite{10.1145/3219819.3220087} propose a causal framework for direct and indirect discrimination in rankings. They propose a definition for direct and indirect discrimination and also propose a post-processing algorithm based on a quadratic program to obtain a fair ranking where the input is a ranked list, not estimated relevance scores. In order to build a causal graph for ranked data, they first use the MLE of the Bradley-Terry-Luce model to estimate scores for each item and then use the score random variable as a node in the causal graph. They define direct (indirect) discrimination in terms of the direct (indirect) path specific effect from the sensitive feature to the score node.

==> amanda/to_do.tex <==
ToDo:
1. Review other approaches to ranking (besides the policy learning approach).
2. Review notions of distance on rankings. In particular, pay attention to distances that account for exposure and relevance.
3. Work out the details of SENSR/SENSEI with the optimal transport metric on candidate sets. 
- If relevance scores are inflated for one group, can our method correct for this?
4. Look for datasets

==> fair-ranking%20(ICLR%202021)/YK-macros.tex <==

\def\Avar{{\sf Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{{\sf aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{{\sf avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{{\sf bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{{\sf Ber}}
\def\bin{{\sf bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{{\sf cat}}
\def\Cov{{\sf Cov}}
\def\cov{{\sf cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{{\sf cl}}
\def\complex{{\bbC}}
\def\cone{{\sf cone}}
\def\conv{{\sf conv}}
\def\deq{\overset{d}{=}}
\def\det{{\sf det}}
\def\diag{{\sf diag}}
\def\diam{{\sf diam}}
\def\dist{{\sf dist}}
\def\dom{{\sf dom}}
\def\doop{{\sf do}}
\def\dto{\overset{\sf d}{\to}}
\def\Ex{{\bbE}}
\def\Exp{{\sf Exp}}
\def\exp{{\sf exp}}
\def\eg{{\it e.g.}}
\def\epi{{\sf epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\iid{{\sf iid}}
\def\ind{{\sf ind}}
\def\intr{{\sf int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{{\sf KL}}
\def\ker{{\sf ker}}
\def\lspan{{\sf span}}
\def\maximize{{\sf maximize}}
\def\med{{\sf med}}
\def\minimize{{\sf minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{{\sf Poi}}
\def\Pr{{\bbP}}
\def\peq{\overset{\sf p}{=}}
\def\plim{{\sf plim}}
\def\proj{{\sf proj}}
\def\prox{{\sf prox}}
\def\pto{\overset{\sf p}{\to}}
\def\ran{{\sf ran}}
\def\rank{{\sf rank}}
\def\reals{{\bbR}}
\def\relint{{\sf relint}}
\def\sign{{\sf sign}}
\def\supp{{\sf supp}}
\def\symm{{\bbS}}

\def\st{\textrm{subject to}}
\def\tr{{\sf tr}}
\def\tube{{\sf tube}}
\def\TV{{\sf TV}}
\def\unif{{\sf unif}}
\def\Var{{\sf Var}}
\def\var{{\sf var}}
\def\vct{{\sf vec}}
\def\veps{\varepsilon}
\def\vol{{\sf vol}}
\def\zeros{\mathbf{0}}


==> fair-ranking%20(ICLR%202021)/YK-thm-macros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}


==> fair-ranking%20(ICLR%202021)/amanda/data.tex <==
1. Yahoo Learning to Rank: http://proceedings.mlr.press/v14/chapelle11a/chapelle11a.pdf?

2. W3C experts in \cite{DBLP:journals/corr/abs-1805-08716}, need to request. They inferred gender by looking at the name manually and injected bias by placing qualified men before qualified women. But then I don't understand how they estimated the probability that a document is in the first position, unless the probability is either 1 or 0. 

3. Engineering Student data set in \cite{DBLP:journals/corr/abs-1805-08716}, need to request. They turned it into a LTR dataset by sorting by grade.

4. Law Students Data set in \cite{DBLP:journals/corr/abs-1805-08716}. They turned it into a LTR dataset.

5. XING Data set in \cite{zehlike2017fa}. ``XING is a career-oriented website from which we automatically collected the top-40 profiles returned for 54 queries, using three for which there is a clear difference between top-10 and top-40. We used a non-personalized (not logged in) search interface and confirmed that it yields the same results from different locations. For each profile, we collected gender, list of positions held, list of education details, and the number of times each profile has been viewed in the platform, which is a measure of popularity of the profile. With this information, we constructed an ad-hoc score: the months of work experience plus the months of education, multiplied by the number of views of the profile. This score tends to be somewhat higher for profiles in the first positions of the search results, but in general does not approximate the proprietary ordering in which profiles are shown. We include this score and its components in our anonymized data release. We use the appropriate gender for each query as the protected group." Code and data: https://github.com/MilkaLichtblau/FA-IR_Ranking

6. Airbnb dataset used in \cite{biega2018equity}. http://insideairbnb.com/

7. Stackexchange data set used in \cite{biega2018equity}

8. TREC 2019 Fair Ranking Track \cite{biega2020overview}: The data is based on Semantic Scholar searches.
- paper data: paper ID, title, abstract, authors (resolved to author IDs), inbound and outbound citations, sensitive feature is whether or not authors are from an advanced economy country, developing, or mixed (ie authors from both advanced and developing country)
- query data: query string, query normalized frequency, a list of documents with number of clicks each document gets (only 6 documents per query, unless the documents presented for a given query change over time and I’m not sure if the documents are ordered or just presented as a set), binary relevance (if a document was clicked or not)
- lots of issues: click rate could be biased, binary relevance, can’t use gender, the fact that it’s only 6 documents might make it trivial


==> fair-ranking%20(ICLR%202021)/amanda/intro.tex <==
Ranking systems are ubiquitous.

\cite{geyik2019fairness} empirically showed that LinkedIn queries are not group fair. Interestingly, they showed that group fairness does not necessarily harm business metrics.

==> fair-ranking%20(ICLR%202021)/amanda/related_work_summary.tex <==
%Another line of work models the amount of exposure documents receive at each position in the ranking and allocates exposure based on this exposure model and document relevance \cite{singh2018Fairness, DBLP:journals/corr/abs-1805-08716, biega2018equity, singh2019Policy}. These works consider both group and individual fairness settings. \cite{DBLP:journals/corr/abs-1805-08716} learns a group fair LTR system that gives the minority group at least as much as exposure as the majority group. Similarly, \cite{singh2019Policy}, which builds on the post-processing work of \cite{singh2018Fairness}, learns a group fair or individually fair LTR system using a similar constraint that also takes relevance into account. \cite{biega2018equity} considers the online setting and proposes a post processing algorithm to obtain an individually fair LTR system by requiring that the ratio of cumulative attention to cumulative relevance is equal for each document.

\cite{StoyanovichAndYang} propose three group fairness measures. In their set-up, they assume a binary protected attribute. However, they do not assume a relevance score of each item, so their notions of fairness are not tied to any notion of accuracy. Their first two metrics define a fair ranking as a ranking that for the first $k$ positions in the ranking for $k \in [k_1, k_2, ...]$, the proportion of individuals from the majority/minority group is approximately equal to the proportion of majority/minority in the whole population. Their metrics put more importance of the proportions being equal for smaller $k$. The difference between the first two metrics is one is differentiable version of the other. Their third metric looks at the ratio of the majority to the minority in the top $k$ compared to the ratio of the majority to the minority. This paper is mostly about proposing metrics, not learning a fair ranking system although they do have some preliminary experiments by using their definitions of fairness as regularizer. 

\cite{DBLP:journals/corr/abs-1805-08716} propose a list-wise fair LTR algorithm: DELTR (Disparate Exposure in Learning to Rank). They claim that they are the first to propose an in-processing fair LTR algorithm. They assume that each document belongs to a minority or majority group. Their notion of fairness borrows from the definition of exposure in \cite{singh2018fairness}: \[\mathrm{Exposure}(d|P) = \sum_{i=1}^n P_{d,j} v_j\] where $d$ is a document, $P_{d,j}$ is the probability that $d$ is ranked in position $j$, and $v_j$ is the position bias of position $j$ ($v_j = \frac{1}{\log(1+j)}$). However, they only consider the case when $j = 1$ because their loss function only depends on the probability of a document being ranked first. They use a group notion of fairness: for each query, the average exposure documents from the minority group receive should equal or exceed the exposure that documents from the majority group receive. They incorporate this fairness constraint as a regularizer to the ListNet objective. 

%But how do you compute the empirical probability that a document is the first? With the relevance scores? What does the data for their real experiments look like? For the engineering student data set, are there only like 16 training samples and 4 testing samples?

\cite{zehlike2017fa} they propose a definition of group fairness for rankings, give a statistical test for determining if a ranking is fair, and propose a post-processing method to obtain a fair ranking. Post-processing means that they do not learn scores for each document and use the relevance scores given to them, i.e. they do not learn a ranking system which can take as input new queries/documents and predict new rankings. Their notion of fairness ``is based on ensuring that the proportion of protected candidates in every prefix of the top-$k$ ranking remains statistically above or indistinguishable from a given minimum." They assume a binary protected attribute. Their post-processing algorithm is a greedy algorithm to produce a top-$k$ fair ranking by separately sorting the majority/minority group into two lists based on relevance scores. Based on their statistical test, for each $t \in [k]$, there must be at least $p_t$ minority individuals in the top $t$ of the ranking. Therefore, to pick the $t$-th individual in the ranking of size $k$, they either pick the best individual remaining from the union of the majority/minority lists or they must pick the best individual remaining from the minority list if the number of minority individuals will not exceed $p_t$.

\cite{biega2018equity} proposes an individually fair definition of fairness in rankings: amortized over multiple queries, the attention (measured by the position in the ranking) each document receives should be proportional to its relevance. They refer to this definition is \textit{equity of attention}. This is their motivation: ``For example, attention could decrease geometrically, whereas relevance scores may decrease linearly as the rank decreases. If a ranking is displayed unchanged to many searchers over time, the lower-ranked subjects might be systematically and repeatedly disadvantaged in terms of the attention they receive." This is the same idea in \cite{singh2019Policy} except \cite{biega2018equity} consider the individual fairness, online setting. These works were written in parallel. They propose a post-processing algorithm to attain rankings that satisfy amortized individual fairness by considering an online integer linear program (ILP), but they do not propose an efficient or optimal algorithm to solve the ILP.

\cite{DBLP:journals/corr/CelisSV17} consider the problem of finding a utility maximizing ranking subject to upper and lower bounds on the number of documents belonging to a group that appear in the first $k$ positions for $k \in K$. They assume knowledge of the utility that a document in a certain position contributes to a ranking. Their algorithm is a post-processing technique. The main results of their paper are ``fast, exact and approximation algorithms for this constrained ranking maximization problem along with complementary hardness results which, together, give a solid understanding of the computational complexity of this problem." This paper is very TCS and has no experiments.

\cite{singh2018Fairness} propose an exposure based definition of fairness and a post-processing algorithm. In particular, they show how to maximize utility subject to fairness constraints as a linear program where instead of finding a single ranking, they find a distribution of rankings to make the problem feasible. To switch from a single ranking to distributions of rankings, they look at doubly stochastic matrices since every ranking corresponds to a doubly stochastic matrix and vice versa. As the motivation for their exposure based fairness definition, they show that a small difference in relevance can lead to a large difference of exposure, which is particularly important for the application of who to hire for a job. They propose 3 definitions of exposure based fairness. First, demographic parity ensures that the exposure of both groups are equal. Second, disparate treatment ensures the exposure of both groups are proportional to their utility. Third, disparate impact ensures that the click through rates (as a function of exposure) is proportional to utility.

\cite{singh2019Policy} 

\cite{geyik2019fairness} proposes group fair measures very similar to \cite{StoyanovichAndYang}. Their notion of a fair ranking is one whose top $k$ positions contain a certain proportion of individuals from the minority group. The measures they propose are (1) skew\@k and (2) normalized discounted cumulative KL-divergence.  Skew\@k for a sensitive feature is the log of the ratio of the proportion of individuals in the top-k positions with that sensitive feature over the desired proportion.  Normalized discounted cumulative KL-divergence is like normalized discounted cumulative gain except the KL divergence between the distribution of the number of individuals from each sensitive group in the top $k$ positions and the desired distribution is used instead of relevance. They provide a post-processing algorithms, one of which is similar to \cite{zehlike2017fa}. The most interesting thing about this work is that they deployed their algorithm on LinkedIn and found that post-processing the rankings to obtain gender group fair rankings did not effect the quality of the rankings (measured by the number of recruiter messages sent and accepted by candidates) from the user perspective. Group fairness measures were improved 3x and 95\% of all searches had the appropriate gender balance.  

\cite{sapiezynski-2019-fairness} proposes a group fairness metric and a statistical test to audit a ranking for fairness. Their definition/audit depends on the distribution of exposure each sensitive group receives compared to an ideal distribution. Their work is what they claim is a more accurate model of exposure than the model used in \cite{singh2018Fairness, singh2019Policy, biega2018equity}. In particular, they claim that modeling user attention with inverse log weights (i.e. 1/log(i)) is inappropriate because it does not attribute enough attention to the top of the ranking and because it assumes that ``user behavior is the static across all platforms and for all search queries.”

\cite{10.1145/3299869.3300079} work is quite different from the rest. They consider the setting where the ranking function is linear and given by a human. Their goal is to help a human choose positive linear weights that result in quality rankings (ie as close to the original weights that the human gave) yet satisfy fairness constraints given by an oracle. They focus on group fairness but their framework is applicable to arbitrary fairness constraints.

\cite{10.1145/3308558.3313443} propose new definitions of fair rankings that extend beyond exposure and minority representation in the top-k. Their work also addresses the whole ranking instead of just the top-k positions. Their setting is different from the standard LTR setting since they assume their is an underlying ground truth ranking in contrast to relevance scores for the items and their measures use concordant and discordant pairs..``We define a new set of fairness criteria customized for rankings: Rank Equality, Rank Calibration, and Rank Parity based on novel rank-specific error metrics. These criteria are model-agnostic and applicable for many ranking applications, capturing key notions of fairness previously applied only for classification.”  Rank Equality tries to define the false negative rate in classification equivalent for ranking which is a function of discordant pairs where the minority group was incorrectly ranked worse. Rank Calibration of a group tries to define calibration for rankings as a function of the number of discordant pairs where at least one item is from that group. Rank Parity is a function of how many disconcordant pairs ranks an item from one group over another.
discordant

\cite{10.1145/3351095.3372858} consider the scenario where the observed relevance scores for one group is biased, and propose enforcing constraints of the form ``there needs to be at least $\alpha_{k,g}$ individuals from group $g$ in the top $k$ of the ranking.” They assume each item $i$ has a true relevance score $w_i$, but that the observed relevance scores are biased for each group $g$, that is the observed relevance for item $i$ is $\beta_g w_i$, where $\beta_g \geq 0$. Their goal is to find a ranking that maximizes utility as a function of the true relevance scores. Theoretically, they have three results. First, they show that there always exists constraints (i.e. minimums on the number of individuals from group $g$ in the top $k$ positions) so that the ranking that maximizes the constrained problem based on the observed biased relevance scores equals the ranking that maximizes the utility based on the true relevance scores. However, these constraints require knowing the bias, i.e. $\beta_g$. Second, they show that if the relevance scores for both groups are drawn from the same continuous distribution, then with high probability the optimal ranking based on the true relevances scores puts $k \frac{m_a}{m_a m_b}$ individuals from the minority group in the top k positions where $m_a$ is the number of minority items and $m_b$ is the number of majority candidates. This motivates enforcing a ``Rooney Rule” type of constraint, i.e. require that at least $k \frac{m_a}{m_a m_b}$ of the individuals in the top $k$ come from the minority. Third, assuming that the distribution that the utilities are drawn from is uniform, then maximizing utility subject to the ``Rooney Rule” type of constraints produces a ranking whose utility under the true relevances is close to the utility maximizing ranking based on the true, unbiased relevances.

\cite{0d8212cdb710458e9a32312c0ffe3a11} consider the problem of group fairness when each person can belong to more than one group. Their notion of fairness is that anyone in the top $k$ from group $g$ must have a higher relevance than anyone not in the top $k$ in group $g$. There exists cases when maximizing utility subject to fairness (what they call diversity) constraints of the form “there must be at least $\alpha_{k,g}$ of people from group $g$ in the top $k$ for the ranking” results in a ranking that violates this notion of fairness. See their example 1. This cannot happen with just two groups (e.g. male and female). They propose an integer program to find a ranking that satisfies both their notion of fairness and diversity constraints.

\cite{10.1145/3219819.3220087} propose a causal framework for direct and indirect discrimination in rankings. They propose a definition for direct and indirect discrimination and also propose a post-processing algorithm based on a quadratic program to obtain a fair ranking where the input is a ranked list, not estimated relevance scores. In order to build a causal graph for ranked data, they first use the MLE of the Bradley-Terry-Luce model to estimate scores for each item and then use the score random variable as a node in the causal graph. They define direct (indirect) discrimination in terms of the direct (indirect) path specific effect from the sensitive feature to the score node.

==> fair-ranking%20(ICLR%202021)/amanda/to_do.tex <==
ToDo:
1. Review other approaches to ranking (besides the policy learning approach).
2. Review notions of distance on rankings. In particular, pay attention to distances that account for exposure and relevance.
3. Work out the details of SENSR/SENSEI with the optimal transport metric on candidate sets. 
- If relevance scores are inflated for one group, can our method correct for this?
4. Look for datasets

==> fair-ranking%20(ICLR%202021)/implicit_feedback_ranking.tex <==
\paragraph{Fair ranking with implicit feedback} In this passage, we change to the notation in Yadav et al \cite{yadav2019Fair}. It is not hard to adapt the preceding approach to ranking with implicit feedback. In ranking with implicit feedback, the relevances are unobserved. Instead, we observe implicit feedback about the relevances of item to a query $c_q\in\{0,1\}$, where $c_q(d) = 1$ indicates relevance (\eg\ user clicks on item) while $c_q(d) = 0$ indicates irrelevance (\eg\ no click). 

The main issue in this partial information setting is it is not possible to evaluate (the empirical counterpart of) the objective in \eqref{eq:utility-maximization}. To circumvent this issue, we replace the utility maximization objective with an estimate:
\[
\widehat{U}(\pi\mid q) \triangleq \Ex_{r\sim\pi(\cdot\mid q)}\big[\hDelta(r,c_q)\big],
\]
where $\hDelta(r,c_q)$ is an estimate of $\Delta(r,\rel^q)$. To keep things simple, we assume the ranking metric is additive:
\[
\Delta(r,\rel^q) = \sum_{d\in d^q}f(r(d))\cdot\rel_q(d),
\]
where $r(d)$ is the rank of item $d$ and $f$ is a weighing function (\eg\ $f(r(d)) = 1/\log_2
(1 + r(d))$ leads to the DCG metric), and the relevances are binary. A basic estimate of the ranking metric is
\[
\hDelta(r,c_q) \triangleq \sum_{d\in d^q}f(r(d))\cdot c_q(d),
\]
but this estimate suffers from \textbf{presentation bias} because users are more likely to click on highly ranked items. To debias the basic estimate, we weigh the implicit feedback by a \textbf{propensity score}. Let $o_q(d)\in\{0,1\}$ indicate whether the user saw item $d$. The propensity score $\Pr(o_q(d) = 1\mid r_q)$ is the ``propensity'' of the user presented with ranking $r_q$ seeing item $d$, and the \textbf{inverse propensity score (IPS)} estimate of the ranking metric is 
\[
\hDelta(r,c_q) \triangleq \sum_{d\in d^q}f(r(d))\cdot\frac{c_q(d)}{\Pr(o_q(d) = 1\mid r_q)}.
\]
As long as the propensity scores are bounded away from zero, it is possible to show that $\hDelta(r,c_q)$ is an unbiased estimate of $\Delta(r,\rel^q)$ \cite{joachims2017Unbiased}, so $\widehat{U}(\pi\mid q)$ is an unbiased estimate of $U(\pi\mid q)$. 

There are many ways to model the propensity score. The most common and simplest model is a rank-based model in which $\Pr(o_q(d) = 1\mid r_q)$ depends on only the rank of $d$ in the ranking $r_q$ presented during logging:
\[
\Pr(o_q(d) = 1\mid r_q) = v(r_q(d))\text{ for some non-increasing }v:\bN\to\bR.
\]
There are also more sophisticated models that depend on contextual information \cite{fang2019Intervention}. It is possible to fit both models with swap experiments \cite{joachims2017Unbiased} or intervention harvesting \cite{agarwal2019Estimating,fang2019Intervention}.



==> fair-ranking%20(ICLR%202021)/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> fair-ranking%20(ICLR%202021)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> fair-ranking%20(ICLR%202021)/rebuttal.tex <==
We thank all the reviewers for their thoughtful comments. We answer each reviewer’s questions individually, and we have updated the draft according to the feedback and suggestions.
---------------------
AnonReviewer1:

Thank you for your feedback. To make our paper better self-contained, we included the precise statement of Theorem 2.3 of Yurochkin & Sun 2020. We address your questions and comments below.

1. "however the maths are hard to follow and little intuition is given. I didn't find an explanation of how the counterfactuals are computed."

There are two places where counterfactuals are used: SenSTIR and the evaluation metric for individual fairness in the experiments. 

Regarding SenSTIR and counterfactuals, Line 3 in Algorithm 1 is where the counterfactuals are computed in SenSTIR. For each query q_{t_i} in the minibatch, we find its counterfactual q_{t_i}' by maximizing the given optimization problem. This optimization problem is the dual of the fair regularizer in eq. 2.4 (please see a discussion after eq. 2.4 for the intuition behind the regularizer).

To evaluate individual fairness in our experiments, we quantify if the LTR system produces similar ranking distributions for a query and its counterfactual. For the German experiments, for every test query, we create a counterfactual that consists of the same set of people as the test query except each person's gender is flipped. For the Microsoft learning-to-rank experiments, for every test query q', we find the closest query q in the training and testing set such that q' \neq q and where the distance is with respect to the fair metric on queries.

2. "just "flipping" the gender is hardly enough as gender is correlated to all others attributes."

 First, this example we use throughout the paper to explain SenSTIR at a high-level is simplistic for the sake of illustration. In general and in our real data experiments, the counterfactual queries that SenSTIR uses in Algorithm 1 can differ from the original query in many ways--not just in one feature--depending on the fair metric. Second, we evaluate the individual fairness properties of the German credit data experiments with \emph{gender} flipped counterfactuals for the sake of intepretability. This evaluation is non-trivial since the fair metric directly deals with \emph{age} information, not gender, so we see how individual fairness can generalize from age to gender. We imagine that ML systems can be unfair to people with respect to features that can be difficult to know before deploying these systems, so although flipping gender is a simplistic choice, it illustrates that SenSTIR can be meaningfully individually fair with respect to these potentially unknown features that were not directly considered when learning the fair metric. 

3. "The legend of figure 3 and 4 are not the same "Kendall's Tau Correlation with Counterfactuals" and "Counterfactual Kendall's Tau Correlation", is it the same metric or something changed ?"

The metric is the same in both cases. Thank you for pointing this out. We have updated the plots. 

4. "In figure 2, Fair-PG-Rank seems to perform very poorly, worse than baseline. As it is the state of the art method, I think some explanation of why it is the case are needed."

Figure 2 shows that Fair-PG-Rank does not necessarily produce individually fair LTR systems. Fair-PG-Rank was made to achieve group--not individual--fairness in LTR systems, so this finding is not surprising. 

5. "Finally most of the paper is based on work done in Yurochkin & Sun 2020 and Yurochkin et al 2020. I think that the authors should explicit the link between the current paper and those two citations." 

We have already commented on the connection between SenSTIR and Yurochkin & Sun 2020 and Yurochkin et al. 2020 in the main text. See the paragraph after Equation 2.4. Please let us know if there is something more specific you would like us to elaborate on. To summarize, we cannot simply apply these prior works in the LTR setting because of two non-trivial challenges: (i) defining a fair distance on queries, i.e., sets of items, and (ii) ensuring the resulting optimization problem is differentiable. Regarding the first challenge, recall that individual fairness requires that similar inputs be treated similarly. Similarity of inputs is quantified by a fair metric. In the LTR setting, the inputs are queries, i.e. sets of items, so we must define a meaningful distance on sets. This challenge is resolved at the end of Section 2.1. Regarding the second challenge, we need to ensure the resulting optimization problem, which depends on the fair metric on queries, is differentiable to make learning possible. This challenge is resolved in Section 3.

----------------------------
AnonReviewer2:

Thank you for your feedback. We replaced the word “sufficient” with "adequate" and cleaned-up the references. We address your comments and questions below.

1. “One question I had is how this would generalize to multiple sensitive features?” 

SenSTIR enforces individual fairness, which depends on a fair metric instead of protected groups (indicated by one or many sensitive features). It is certainly possible to define a fair metric in a way that encodes the intersectional invariances from multiple protected groups/sensitive features (e.g. Yurochkin et al. 2020, Mukherjee et al. 2020), and SenSTIR will enforce these invariances. 

2. “Can the authors say something about computational complexity? Is the problem 2.4 NP-hard? Is Algorithm 1 an approximation? What is the running time of Algorithm 1 both in theory and in the experiments (seconds). How does the running time of SenSTIR compare with Fair-PG-Rank?”

Equation 2.4 as written is hard to solve, but the dual is solvable for convex losses. However, if the ranking policies \pi are parameterized by a neural net, then in general problem 2.4 is non-convex. Finding the optimum of non-convex problems is typically NP-hard, yet solving non-convex problems like those in deep learning is still tremendously valuable and practically feasible.   

For the German experiments, SenSTIR takes 19.2 minutes, and the average time for each epoch of Algorithm 1 is 0.06 seconds with a standard deviation of 0.016 seconds. Using the implementation of Fair-PG-Rank provided by the authors (found at https://github.com/ashudeep/Fair-PGRank), Fair-PG-Rank takes 73.31 minutes, and the average time for each epoch is 43.98 seconds with a standard deviation of 5.61 seconds. We believe that the run times of both of these algorithms can be significantly improved with optimizations to the code.

3. “A higher level question is why the authors did not test fair supervised learning algorithms. (I didn't quite understand the point about not defining a distance on sets.)”

At a high level, individual fairness says that an ML system should produce similar outputs for similar inputs (where similarity is measured by the fair metric). As you noted, measuring the similarity of outputs in SL can be generalized to LTR (i.e. measuring the similarity of relevance scores). However, measuring the similarity of inputs in LTR is different. The inputs to the LTR problem are sets of items (i.e. unordered collections of feature vectors), while in SL the inputs are singleton feature vectors. In other words, individual fairness for LTR should intuitively imply similar ranking outputs on similar sets of items, therefore requiring a fair metric on sets. In other words, it is the set, not individual items that matter here. This difference prevents us from being able to apply fair supervised learning methods directly. Another important difference between LTR and SL is the loss function, as you noted.

-----------------------------
AnonReviewer3: [Thank you for your feedback. However, some of the criticism is due to misunderstandings.]

We thank you for your feedback, and address your comments below.

1. "A practical objection to the approach is the use of randomized rankers to get around the important issue that ranking is by its very nature unfair to individuals."

First, stochastic ranking policies are a way to make the LTR problem feasible. Otherwise, searching for utility-maximizing rankings would take time that is exponential in the query size. This is also something that is standard in the literature on fair ranking (see Biega et al 2018, Singh & Joachims 2018, 2019, and Zehlike & Castillo 2020). 

Second, we wish to point out that when we evaluate the individual fairness of our ranking policies, we are not averaging over many draws from the ranking policy. In particular, when we evaluate individual fairness by comparing the distance between the ranking of a query and the ranking of its counterfactual query, we use the deterministic rankings given by sorting the items by their predicted scores, instead of drawing rankings from the learned distributions.

Third, while the long-term effects of ranking policies are interesting, they are difficult to study because the results are very sensitive to the exact model for how the ranking policy affects the state of the system. This is also a very different problem than the problem that we address in this paper. We now mention the paper you referenced in the conclusion.

2. "I just can't find a proper metric for individual fairness in the paper. The only proposal is a comparison between the outputs of the ranker before and after altering some features fed into it."

This statement is not true. We only use this evaluation for the German credit experiments. We evaluate individual fairness in the synthetic and the Microsoft LTR experiments quite differently as stated in the second paragraph of the "Results" paragraph of Section 5.1 and in the "Comparison metrics" paragraph in Section 5.3. In particular, for the Microsoft experiments, for every query q in the test set, we find the closest query $q'$ in the train and test set such that $q' \neq q$ where the distance is with respect to the fair metric. Then we compare the outputs of the ranker on $q$ and $q'$. We can think of $q'$ as a counterfactual that exists in the data. 

3. "This way of evaluating rankers makes no sense to me at all because a really easy way for a ranker to appear fair is by not using the feature being modified (e.g. age or gender) directly, but inferring it from the remaining features. I think the issue is that the authors are confused by the subtle but crucially important distinction between losses and metrics. You're allowed to use whatever information you like when you're designing your loss, but the final evaluation should not rely on the model, but just its output."

We think that the reviewer misunderstood the evaluation metrics. We agree that the final evaluation should not rely on the model - and that is what we did in our evaluation when flipping the gender feature in the German experiments, a feature not given special consideration when training SenSTIR or learning a fair metric. We provide a more detailed justification of this choice below.

We use this evaluation metric on the German credit experiments since it is (1) easily interpretable, (2) non-trivial, and (3) is standard in the literature. First, individual fairness means that pairs of similar inputs, i.e. queries, should be treated similarly. One interpretable way to check this notion of fairness is to see if two queries of people that differ only with respect to gender are ranked similarly.

Second, this evaluation metric is non-trivial for the German credit experiments since the fair metric is trained to ignore variation in the data due to *age*, but we evaluate individual fairness with respect to *gender*. We imagine that ML systems can be unfair to people with respect to features that can be difficult to know before deploying these systems, so although flipping gender is a simplistic choice, it illustrates that SenSTIR can be meaningfully individually fair with respect to these potentially unknown features that were not given special consideration when choosing the fair metric or in training with SenSTIR. In addition, the "Project" baseline (see the "Baselines" paragraph in the beginning of Section 5) does not use age as a feature yet it is significantly not individually fair with respect to counterfactual queries obtained by flipping the gender of each person.

Third, our evaluation metric for individual fairness in the German credit experiments is the natural analogue of what is standard in the individual fairness literature for classification (Yurochkin et al. 2020, Yurochkin & Sun 2020, Garg et al. 2018). We are open to suggestions of other evaluation metrics.

4. Comparison to LambdaMART

First, the point of our paper is not to beat the state of the art LTR algorithm, but to demonstrate how to achieve individual fairness in the LTR setting since prior work has mostly focused on group fair LTR systems. Nonetheless, Singh & Joachims 2019 have experiments demonstrating that stochastic policy rankers (i.e. SenSTIR when the fair regularization \rho = 0) produces rankers that are competitive with other LTR baselines.

Second, LambdaMART is a boosted tree-based method, so neither our method nor prior work like Singh & Joachims 2019 is applicable since these methods require a differentiable objective. However, we think that coming up with an individually fair version of LambdaMART is an interesting line of future work. 

-----------------------------
AnonReviewer4:
Thank you for your feedback to improve our paper, and we fixed the bibliography as you pointed out. We address your question and comment below.

1. "My only question for the authors is how easy would it be to learn fair metric in a typical application for LTR models?"

One major contribution of our work is showing how to obtain a fair metric on queries--needed in order to use SenSTIR--from a fair metric on item representations via optimal transport tools. See the end of Section 2.1. In our real data experiments, we showed that it is possible to learn effective fair metrics in the LTR setting based off the prior techniques for fair metric learning designed for regression/classification (Yurochkin et al. 2020, Mukherjee et al. 2020). Hence, in the future, SenSTIR can utilize new methods that are not necessarily intended for the LTR setting for learning fair metrics.

2. "On page 4 section 3 authors reference Theorem 2.3 but in the citation there is no Theorem 2.3."

Theorem 2.3 of "SenSeI: Sensitive Set Invariance for Enforcing Individual Fairness" by Yurochkin & Sun 2020 (https://arxiv.org/pdf/2006.14168.pdf) can be found at the top of page 4 in their paper. We have also added the statement of this theorem to section 3 of our paper for completeness.




==> implicit_feedback_ranking.tex <==
\paragraph{Fair ranking with implicit feedback} In this passage, we change to the notation in Yadav et al \cite{yadav2019Fair}. It is not hard to adapt the preceding approach to ranking with implicit feedback. In ranking with implicit feedback, the relevances are unobserved. Instead, we observe implicit feedback about the relevances of item to a query $c_q\in\{0,1\}$, where $c_q(d) = 1$ indicates relevance (\eg\ user clicks on item) while $c_q(d) = 0$ indicates irrelevance (\eg\ no click). 

The main issue in this partial information setting is it is not possible to evaluate (the empirical counterpart of) the objective in \eqref{eq:utility-maximization}. To circumvent this issue, we replace the utility maximization objective with an estimate:
\[
\widehat{U}(\pi\mid q) \triangleq \Ex_{r\sim\pi(\cdot\mid q)}\big[\hDelta(r,c_q)\big],
\]
where $\hDelta(r,c_q)$ is an estimate of $\Delta(r,\rel^q)$. To keep things simple, we assume the ranking metric is additive:
\[
\Delta(r,\rel^q) = \sum_{d\in d^q}f(r(d))\cdot\rel_q(d),
\]
where $r(d)$ is the rank of item $d$ and $f$ is a weighing function (\eg\ $f(r(d)) = 1/\log_2
(1 + r(d))$ leads to the DCG metric), and the relevances are binary. A basic estimate of the ranking metric is
\[
\hDelta(r,c_q) \triangleq \sum_{d\in d^q}f(r(d))\cdot c_q(d),
\]
but this estimate suffers from \textbf{presentation bias} because users are more likely to click on highly ranked items. To debias the basic estimate, we weigh the implicit feedback by a \textbf{propensity score}. Let $o_q(d)\in\{0,1\}$ indicate whether the user saw item $d$. The propensity score $\Pr(o_q(d) = 1\mid r_q)$ is the ``propensity'' of the user presented with ranking $r_q$ seeing item $d$, and the \textbf{inverse propensity score (IPS)} estimate of the ranking metric is 
\[
\hDelta(r,c_q) \triangleq \sum_{d\in d^q}f(r(d))\cdot\frac{c_q(d)}{\Pr(o_q(d) = 1\mid r_q)}.
\]
As long as the propensity scores are bounded away from zero, it is possible to show that $\hDelta(r,c_q)$ is an unbiased estimate of $\Delta(r,\rel^q)$ \cite{joachims2017Unbiased}, so $\widehat{U}(\pi\mid q)$ is an unbiased estimate of $U(\pi\mid q)$. 

There are many ways to model the propensity score. The most common and simplest model is a rank-based model in which $\Pr(o_q(d) = 1\mid r_q)$ depends on only the rank of $d$ in the ranking $r_q$ presented during logging:
\[
\Pr(o_q(d) = 1\mid r_q) = v(r_q(d))\text{ for some non-increasing }v:\bN\to\bR.
\]
There are also more sophisticated models that depend on contextual information \cite{fang2019Intervention}. It is possible to fit both models with swap experiments \cite{joachims2017Unbiased} or intervention harvesting \cite{agarwal2019Estimating,fang2019Intervention}.



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> rebuttal.tex <==
We thank all the reviewers for their thoughtful comments. We answer each reviewer’s questions individually, and we have updated the draft according to the feedback and suggestions.
---------------------
AnonReviewer1:

Thank you for your feedback. To make our paper better self-contained, we included the precise statement of Theorem 2.3 of Yurochkin & Sun 2020. We address your questions and comments below.

1. "however the maths are hard to follow and little intuition is given. I didn't find an explanation of how the counterfactuals are computed."

There are two places where counterfactuals are used: SenSTIR and the evaluation metric for individual fairness in the experiments. 

Regarding SenSTIR and counterfactuals, Line 3 in Algorithm 1 is where the counterfactuals are computed in SenSTIR. For each query q_{t_i} in the minibatch, we find its counterfactual q_{t_i}' by maximizing the given optimization problem. This optimization problem is the dual of the fair regularizer in eq. 2.4 (please see a discussion after eq. 2.4 for the intuition behind the regularizer).

To evaluate individual fairness in our experiments, we quantify if the LTR system produces similar ranking distributions for a query and its counterfactual. For the German experiments, for every test query, we create a counterfactual that consists of the same set of people as the test query except each person's gender is flipped. For the Microsoft learning-to-rank experiments, for every test query q', we find the closest query q in the training and testing set such that q' \neq q and where the distance is with respect to the fair metric on queries.

2. "just "flipping" the gender is hardly enough as gender is correlated to all others attributes."

 First, this example we use throughout the paper to explain SenSTIR at a high-level is simplistic for the sake of illustration. In general and in our real data experiments, the counterfactual queries that SenSTIR uses in Algorithm 1 can differ from the original query in many ways--not just in one feature--depending on the fair metric. Second, we evaluate the individual fairness properties of the German credit data experiments with \emph{gender} flipped counterfactuals for the sake of intepretability. This evaluation is non-trivial since the fair metric directly deals with \emph{age} information, not gender, so we see how individual fairness can generalize from age to gender. We imagine that ML systems can be unfair to people with respect to features that can be difficult to know before deploying these systems, so although flipping gender is a simplistic choice, it illustrates that SenSTIR can be meaningfully individually fair with respect to these potentially unknown features that were not directly considered when learning the fair metric. 

3. "The legend of figure 3 and 4 are not the same "Kendall's Tau Correlation with Counterfactuals" and "Counterfactual Kendall's Tau Correlation", is it the same metric or something changed ?"

The metric is the same in both cases. Thank you for pointing this out. We have updated the plots. 

4. "In figure 2, Fair-PG-Rank seems to perform very poorly, worse than baseline. As it is the state of the art method, I think some explanation of why it is the case are needed."

Figure 2 shows that Fair-PG-Rank does not necessarily produce individually fair LTR systems. Fair-PG-Rank was made to achieve group--not individual--fairness in LTR systems, so this finding is not surprising. 

5. "Finally most of the paper is based on work done in Yurochkin & Sun 2020 and Yurochkin et al 2020. I think that the authors should explicit the link between the current paper and those two citations." 

We have already commented on the connection between SenSTIR and Yurochkin & Sun 2020 and Yurochkin et al. 2020 in the main text. See the paragraph after Equation 2.4. Please let us know if there is something more specific you would like us to elaborate on. To summarize, we cannot simply apply these prior works in the LTR setting because of two non-trivial challenges: (i) defining a fair distance on queries, i.e., sets of items, and (ii) ensuring the resulting optimization problem is differentiable. Regarding the first challenge, recall that individual fairness requires that similar inputs be treated similarly. Similarity of inputs is quantified by a fair metric. In the LTR setting, the inputs are queries, i.e. sets of items, so we must define a meaningful distance on sets. This challenge is resolved at the end of Section 2.1. Regarding the second challenge, we need to ensure the resulting optimization problem, which depends on the fair metric on queries, is differentiable to make learning possible. This challenge is resolved in Section 3.

----------------------------
AnonReviewer2:

Thank you for your feedback. We replaced the word “sufficient” with "adequate" and cleaned-up the references. We address your comments and questions below.

1. “One question I had is how this would generalize to multiple sensitive features?” 

SenSTIR enforces individual fairness, which depends on a fair metric instead of protected groups (indicated by one or many sensitive features). It is certainly possible to define a fair metric in a way that encodes the intersectional invariances from multiple protected groups/sensitive features (e.g. Yurochkin et al. 2020, Mukherjee et al. 2020), and SenSTIR will enforce these invariances. 

2. “Can the authors say something about computational complexity? Is the problem 2.4 NP-hard? Is Algorithm 1 an approximation? What is the running time of Algorithm 1 both in theory and in the experiments (seconds). How does the running time of SenSTIR compare with Fair-PG-Rank?”

Equation 2.4 as written is hard to solve, but the dual is solvable for convex losses. However, if the ranking policies \pi are parameterized by a neural net, then in general problem 2.4 is non-convex. Finding the optimum of non-convex problems is typically NP-hard, yet solving non-convex problems like those in deep learning is still tremendously valuable and practically feasible.   

For the German experiments, SenSTIR takes 19.2 minutes, and the average time for each epoch of Algorithm 1 is 0.06 seconds with a standard deviation of 0.016 seconds. Using the implementation of Fair-PG-Rank provided by the authors (found at https://github.com/ashudeep/Fair-PGRank), Fair-PG-Rank takes 73.31 minutes, and the average time for each epoch is 43.98 seconds with a standard deviation of 5.61 seconds. We believe that the run times of both of these algorithms can be significantly improved with optimizations to the code.

3. “A higher level question is why the authors did not test fair supervised learning algorithms. (I didn't quite understand the point about not defining a distance on sets.)”

At a high level, individual fairness says that an ML system should produce similar outputs for similar inputs (where similarity is measured by the fair metric). As you noted, measuring the similarity of outputs in SL can be generalized to LTR (i.e. measuring the similarity of relevance scores). However, measuring the similarity of inputs in LTR is different. The inputs to the LTR problem are sets of items (i.e. unordered collections of feature vectors), while in SL the inputs are singleton feature vectors. In other words, individual fairness for LTR should intuitively imply similar ranking outputs on similar sets of items, therefore requiring a fair metric on sets. In other words, it is the set, not individual items that matter here. This difference prevents us from being able to apply fair supervised learning methods directly. Another important difference between LTR and SL is the loss function, as you noted.

-----------------------------
AnonReviewer3: [Thank you for your feedback. However, some of the criticism is due to misunderstandings.]

We thank you for your feedback, and address your comments below.

1. "A practical objection to the approach is the use of randomized rankers to get around the important issue that ranking is by its very nature unfair to individuals."

First, stochastic ranking policies are a way to make the LTR problem feasible. Otherwise, searching for utility-maximizing rankings would take time that is exponential in the query size. This is also something that is standard in the literature on fair ranking (see Biega et al 2018, Singh & Joachims 2018, 2019, and Zehlike & Castillo 2020). 

Second, we wish to point out that when we evaluate the individual fairness of our ranking policies, we are not averaging over many draws from the ranking policy. In particular, when we evaluate individual fairness by comparing the distance between the ranking of a query and the ranking of its counterfactual query, we use the deterministic rankings given by sorting the items by their predicted scores, instead of drawing rankings from the learned distributions.

Third, while the long-term effects of ranking policies are interesting, they are difficult to study because the results are very sensitive to the exact model for how the ranking policy affects the state of the system. This is also a very different problem than the problem that we address in this paper. We now mention the paper you referenced in the conclusion.

2. "I just can't find a proper metric for individual fairness in the paper. The only proposal is a comparison between the outputs of the ranker before and after altering some features fed into it."

This statement is not true. We only use this evaluation for the German credit experiments. We evaluate individual fairness in the synthetic and the Microsoft LTR experiments quite differently as stated in the second paragraph of the "Results" paragraph of Section 5.1 and in the "Comparison metrics" paragraph in Section 5.3. In particular, for the Microsoft experiments, for every query q in the test set, we find the closest query $q'$ in the train and test set such that $q' \neq q$ where the distance is with respect to the fair metric. Then we compare the outputs of the ranker on $q$ and $q'$. We can think of $q'$ as a counterfactual that exists in the data. 

3. "This way of evaluating rankers makes no sense to me at all because a really easy way for a ranker to appear fair is by not using the feature being modified (e.g. age or gender) directly, but inferring it from the remaining features. I think the issue is that the authors are confused by the subtle but crucially important distinction between losses and metrics. You're allowed to use whatever information you like when you're designing your loss, but the final evaluation should not rely on the model, but just its output."

We think that the reviewer misunderstood the evaluation metrics. We agree that the final evaluation should not rely on the model - and that is what we did in our evaluation when flipping the gender feature in the German experiments, a feature not given special consideration when training SenSTIR or learning a fair metric. We provide a more detailed justification of this choice below.

We use this evaluation metric on the German credit experiments since it is (1) easily interpretable, (2) non-trivial, and (3) is standard in the literature. First, individual fairness means that pairs of similar inputs, i.e. queries, should be treated similarly. One interpretable way to check this notion of fairness is to see if two queries of people that differ only with respect to gender are ranked similarly.

Second, this evaluation metric is non-trivial for the German credit experiments since the fair metric is trained to ignore variation in the data due to *age*, but we evaluate individual fairness with respect to *gender*. We imagine that ML systems can be unfair to people with respect to features that can be difficult to know before deploying these systems, so although flipping gender is a simplistic choice, it illustrates that SenSTIR can be meaningfully individually fair with respect to these potentially unknown features that were not given special consideration when choosing the fair metric or in training with SenSTIR. In addition, the "Project" baseline (see the "Baselines" paragraph in the beginning of Section 5) does not use age as a feature yet it is significantly not individually fair with respect to counterfactual queries obtained by flipping the gender of each person.

Third, our evaluation metric for individual fairness in the German credit experiments is the natural analogue of what is standard in the individual fairness literature for classification (Yurochkin et al. 2020, Yurochkin & Sun 2020, Garg et al. 2018). We are open to suggestions of other evaluation metrics.

4. Comparison to LambdaMART

First, the point of our paper is not to beat the state of the art LTR algorithm, but to demonstrate how to achieve individual fairness in the LTR setting since prior work has mostly focused on group fair LTR systems. Nonetheless, Singh & Joachims 2019 have experiments demonstrating that stochastic policy rankers (i.e. SenSTIR when the fair regularization \rho = 0) produces rankers that are competitive with other LTR baselines.

Second, LambdaMART is a boosted tree-based method, so neither our method nor prior work like Singh & Joachims 2019 is applicable since these methods require a differentiable objective. However, we think that coming up with an individually fair version of LambdaMART is an interesting line of future work. 

-----------------------------
AnonReviewer4:
Thank you for your feedback to improve our paper, and we fixed the bibliography as you pointed out. We address your question and comment below.

1. "My only question for the authors is how easy would it be to learn fair metric in a typical application for LTR models?"

One major contribution of our work is showing how to obtain a fair metric on queries--needed in order to use SenSTIR--from a fair metric on item representations via optimal transport tools. See the end of Section 2.1. In our real data experiments, we showed that it is possible to learn effective fair metrics in the LTR setting based off the prior techniques for fair metric learning designed for regression/classification (Yurochkin et al. 2020, Mukherjee et al. 2020). Hence, in the future, SenSTIR can utilize new methods that are not necessarily intended for the LTR setting for learning fair metrics.

2. "On page 4 section 3 authors reference Theorem 2.3 but in the citation there is no Theorem 2.3."

Theorem 2.3 of "SenSeI: Sensitive Set Invariance for Enforcing Individual Fairness" by Yurochkin & Sun 2020 (https://arxiv.org/pdf/2006.14168.pdf) can be found at the top of page 4 in their paper. We have also added the statement of this theorem to section 3 of our paper for completeness.



